Massively Multi-Cultural Knowledge Acquisition & LM Benchmarking

Pretrained large language models have revolutionized many applications but still face challenges related to cultural bias and a lack of cultural commonsense knowledge crucial for guiding cross-culture communication and interactions. Recognizing the shortcomings of existing methods in capturing the diverse and rich cultures across the world, this paper introduces a novel approach for massively multicultural knowledge acquisition. Specifically, our method strategically navigates from densely informative Wikipedia documents on cultural topics to an extensive network of linked pages. Leveraging this valuable source of data collection, we construct the CultureAtlas dataset, which covers a wide range of sub-country level geographical regions and ethnolinguistic groups, with data cleaning and preprocessing to ensure textual assertion sentence self-containment, as well as fine-grained cultural profile information extraction. Our dataset not only facilitates the evaluation of language model performance in culturally diverse contexts but also serves as a foundational tool for the development of culturally sensitive and aware language models. Our work marks an important step towards deeper understanding and bridging the gaps of cultural disparities in AI, to promote a more inclusive and balanced representation of global cultures in the digital domain.

==> notes/about_data.tex <==

% Code: https://github.com/yrf1/CTZL101_MM-NormSage/tree/main

% /data/yifung/CTZL101_MM-NormSage/data/culture_scraped_info/culture_info_beta_Nov21.pkl
%
% # of countries scraped: 194
% # of subcountry regions scraped: 482
% # of subsubcountry geographical regions scraped: 5038
% # of ethno-linguistic groups covered in scrape data: 713
%
% # of pages scraped: 31,030  (fyi there's like 10k state/provinces in the world but not all have detailed wiki pgs)

% ------------------

% Nature of the cultural knowledge (A2)
%
% A


% ------------------


% Reminder of the threads of data file in processing (for faster processing)
% How about keep track of everything w/ culture_info_beta_Nov21_consolidated.pkl
%
% Original Scraping -- culture_info_beta_Nov21_scraped.pkl 
%                   -- fyi this already went through a round of topic filtering by pg tit
% Add Topic Categorization -- culture_info_beta_Nov21_wTopicCat.pkl
%                          -- this is by paragraph, via the extract_frame code (pre_categorize mode)
%                          -- paragraph categorization code execution currently via the categorize_pg() function in src/culture_crawling.py, called on src/extract_NormFrame.py script
%                          -- check % complete:  ?  (utils/print_itmd_proc_stats.py)
% Extract Cultural Profile -- culture_info_beta_Nov21_wCulturalProfile.pkl
%                          -- check the "pg_content_init_norms" field inside the data file
%                          -- check % complete:  ?  (utils/print_itmd_proc_stats.py)
% Generate Negative Versions in Benchmarking -- culture_info_beta_Nov21_wNegVersion.pkl (少量就好)
%                          -- check src/construct_mm_benchmark_beta.py
%
% Cost Estimation -- 

==> sections/3_method.tex <==
\section{Method}

A

==> sections/7_limitations.tex <==
\section{Limitations}
TODO: will write after I do another round of polishing the previous sections

==> tables/5_result_ablation_by_culture_profile.tex <==


\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|}
         \hline 
         \rule{0pt}{1\normalbaselineskip} ~~~~~~~ & ~~~\textbf{Spec.}~~~ & ~~~\textbf{Gen} ~~~\\[0.1cm]
         \hline %\hline
         \rule{0pt}{1\normalbaselineskip} \textbf{Sub-Country Location} & 22.1 & 35.0 \\
         \textbf{Ethnicity} & 27.5 & 35.5 \\
         \textbf{Religion} & 17.9 & 35.0 \\
         \textbf{Marital Status} & 13.7 & 33.6 \\ [0.1cm]
         \hline
    \end{tabular}
    \caption{F-score performance comparison by fine-grained cultural profile framing, such as country-level  vs province-level cultural knowledge.}
    \label{tab:5_result_ablation_by_CultureProfile}
    
\end{table}

==> tables/A1_culture_profile_extraction_performance.tex <==

\begin{table}[!htp]
    \small
    \centering
    \begin{tabular}{p{2.6cm}|c|p{0.38cm}}
         \hline
         \rule{0pt}{\normalbaselineskip} \textbf{Claim Frame Field} & \multirow{2}{3.5cm}{\centering{\textbf{Method}}} & \multirow{2}{0.38cm}{\centering{\textbf{Acc}}} \\
         \centering{\textbf{Parsing Subtask}} & & \\ [0.5ex]
         \hline 
         \multirow{5}{3cm}{\textbf{interactive nature categorization}} & \rule{0pt}{\normalbaselineskip} bart-large-mnli & 0.4 \\ 
          %& RoBERTaQA-large-SQuaD & \\ 
          & Llama2-13B prompting & 0.3 \\
          & ChatGPT prompting & \textbf{0.8} \\
          & GPT4 prompting &  \\ [0.5ex]
          \hline 
          %\multirow{5}{2.5cm}{\textbf{topic categorization}} & \rule{0pt}{\normalbaselineskip} bart-large-mnli & 0.5 \\ 
          %& Llama2-13B prompting & 0.6 \\
          %& ChatGPT prompting & 0.5 \\
          %& GPT4 prompting & 0.5 \\ [0.5ex]
          %\hline 
          \multirow{5}{2.5cm}{\textbf{country-level extraction}} & \rule{0pt}{\normalbaselineskip} UniversalNER & \\ 
          & RoBERTaQA-large-SQuaD & 0.2 \\ 
          & Llama2-13B prompting & \\
          & ChatGPT prompting & \textbf{0.8} \\
          & GPT4 prompting & 0.8 \\ [0.5ex]
          \hline 
          \multirow{5}{3cm}{\textbf{subcountry-level extraction}} & \rule{0pt}{\normalbaselineskip} UniversalNER & \\
          & RoBERTaQA-large-SQuaD & 0.2 \\ 
          & Llama2-13B prompting & \\
          & ChatGPT prompting & \textbf{0.9} \\
          & GPT4 prompting & 0.9 \\ [0.5ex]
          \hline 
          \multirow{5}{2.5cm}{\textbf{ethnicity extraction}} & \rule{0pt}{\normalbaselineskip} UniversalNER & \\ 
          & RoBERTaQA-large-SQuaD & 0.56 \\ 
          & Llama2-13B prompting & \\
          & Llama2-70B prompting & \\
          & ChatGPT prompting & \textbf{0.9} \\ [0.5ex]
          \hline 
          \multirow{5}{3cm}{\textbf{ethnic subgroup extraction}} & \rule{0pt}{\normalbaselineskip} UniversalNER & \\ 
          & RoBERTaQA-large-SQuaD & 0.6 \\ 
          & Llama2-13B prompting & \\
          & Llama2-70B prompting & \\
          & ChatGPT prompting & \\ [0.5ex]
          \hline 
          \multirow{5}{3cm}{\textbf{age extraction}} & \rule{0pt}{\normalbaselineskip} UniversalNER & \\ 
          & RoBERTaQA-large-SQuaD & 0.50 \\ 
          & Llama2-13B prompting & 0.7 \\
          & ChatGPT prompting & \textbf{0.8} \\
          & GPT4 prompting & 0.6 \\ [0.5ex]
          \hline 
          \multirow{5}{3cm}{\textbf{gender extraction}} & \rule{0pt}{\normalbaselineskip} UniversalNER & \\ 
          & RoBERTaQA-large-SQuaD &  0.3 \\ 
          & Llama2-13B prompting & 0.6 \\
          & ChatGPT prompting & \textbf{0.9} \\
          & GPT4 prompting & 0.9 \\ [0.5ex]
          \hline 
          \multirow{5}{3cm}{\textbf{religion belief extraction}} & \rule{0pt}{\normalbaselineskip} UniversalNER & \\ 
          & RoBERTaQA-large-SQuaD & 0.7 \\ 
          & Llama2-13B prompting & \\
          & ChatGPT prompting & \textbf{0.7} \\
          & GPT4 prompting & \\ [0.5ex]
          \hline 
          \multirow{5}{3cm}{\textbf{marital status}} & \rule{0pt}{\normalbaselineskip} UniversalNER & \\ 
          & RoBERTaQA-large-SQuaD & 0.4 \\ 
          & Llama2-13B prompting & \\
          & ChatGPT prompting & \textbf{0.8} \\
          & GPT4 prompting & \\ [0.5ex]
          \hline 
          \multirow{5}{2.5cm}{\textbf{occupation extraction}} & \rule{0pt}{\normalbaselineskip} UniversalNER & \\ 
          & RoBERTaQA-large-SQuaD & 0.33 \\ 
          & Llama2-13B prompting & \\
          & ChatGPT prompting & \textbf{0.7} \\
          & GPT4  prompting & \\ [0.5ex]
          \hline
    \end{tabular}
    \caption{A performance of automatic culture profile extraction in our \textbf{NCLB} benchmark construction process of positive socio-cultural norm discovery.}
    \label{tab:A1_culture_profile_extraction_results}
\end{table}

==> tables/A2_culture_profile_extraction_prompt.tex <==

\begin{table*}[]
    \small 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c}
        \hline
        \rule{0pt}{\normalbaselineskip} \textbf{Culture Profile Field} & \textbf{Directed Question Answering} \\ [0.5ex]
         \hline 
        \rule{0pt}{\normalbaselineskip} interaction nature categorization & Is this an individual human behavioral norm or human-human behavioral norm? \\ [0.5ex]
         topic distribution modeling &  Is this a social norm, cultural norm, belief or ritual, history, politics, or fact? \\ [0.5ex]
         country-level extraction & Which country is mentioned or implied in the sentence? Answer N/A if unknown.\\ [0.5ex]
         sub-country level extraction & Which state/province/city/subcountry region is mentioned \\  [-0.5ex]
         & or implied in the sentence (or answer N/A):\\ [0.5ex]
         ethnicity extraction & Which ethnic group is mentioned or implied in the sentence? \\
         & Answer N/A if unspecified? \\ [0.5ex]
         ethnic subgroup extraction & Which ethnolinguistic subgroup is mentioned or implied in the sentence? \\ [-0.5ex]
         & Answer N/A if unspecified. \\ [0.5ex]
         age extraction & Which age group is mentioned or implied in the sentence? \\ [0.5ex]
         gender extraction & Which gender group is mentioned or implied in the sentence \\ [-0.5ex]
         & (male, female, transgender, or N/A) \\
         marital status & Which marital status is mentioned or implied in the sentence. \\
         religion belief extraction & Which religious group is mentioned or implied in the sentence (or answer N/A): \\ [0.5ex]
         occupation extraction & Which occupation is mentioned or implied in the sentence? \\ [-0.5ex]
         & Answer N/A if unspecified \\
    \end{tabular}
    }
    \caption{Details on the prompt template for cultural profile extraction}
    \label{tab:A2_culture_profile_extraction_prompt}
\end{table*}

==> tables/A4_tab_copy.tex <==

\begin{table*}[!ht]
    \small 
    \centering
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{ccc|ccc|ccc}
        \hline
        \rule{0pt}{\normalbaselineskip} Country 1 & X & X & Country M & X & X & Country Z & x & x\\ [0.5ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        Country 2 & X & X & Country N & X & X & Country X & x & x\\ [0.15ex]
        \hline
    \end{tabular}
    %}
    \caption{The \# of documents and cultural knowledge assertion sentences per culture by ethnolinguistic group}
    \label{tab:A4_data_count_by_ethnolinguistic group}
\end{table*}
